Praxis: Practical Witness Encryption for NP

Witness encryption encrypts a message to an NP statement so that whoever holds a witness can decrypt. Over a decade after its introduction, known constructions for general NP statements are far from practical or rest on heuristic or broken assumptions. We propose Praxis, a practical scheme for NP, and prove it extractable in the bilinear generic group and random oracle models under Module-SIS. Our instantiation encrypts to a Groth16 verifier on BN254, set up honestly, which serves every NP relation at the same cost: at $100$-bit security, its ciphertext is $7.88$ GiB, encryption takes $2^{34.2}$ base-field multiplications, and decryption with a Groth16 proof $2^{33.0}$ on average. We give Lean 4 proofs of correctness and extraction at this instantiation's parameters. Praxis starts from the rank-gap template of the recent feasibility result [Hair and Sahai, arXiv 2026]. Where they raise the gap to keep decryption polynomial, we fix it, so decryption ends with a search that is exponential but concretely fast: $O(2^{\lambda/4} N^{1/4})$ expected operations for a statement in $N$ Boolean unknowns at $\lambda$-bit security. A quadratic arithmetic program makes our hidden matrix low rank, so where their ciphertext encodes a basis of a matrix space, ours holds factors of width two, which a pairing multiplies. Weights and identities from an extension field tie copies of this matrix, so an adversary telling encryptions apart yields a witness or a Module-SIS solution. For the same Groth16 statement and $100$-bit security level, Praxis reduces the ciphertext size and the cost of encryption of either of their constructions by over ten orders of magnitude, and that of decryption by over six.

==> fspdefault.tex <==
%% (C) Antonis Tsolomitis, GPL3.
\setmainfont[%
  SizeFeatures={%
{Size=-8, Font=NewCM08-Book.otf,
      ItalicFont=NewCM08-BookItalic.otf,%
      BoldFont=NewCM10-Bold.otf,%
      BoldItalicFont=NewCM10-BoldItalic.otf,%
      SlantedFont=NewCM08-Book.otf,%
      BoldSlantedFont=NewCM10-Bold.otf,%
      SmallCapsFeatures={Numbers=OldStyle}},
{Size=8, Font=NewCM08-Book.otf,
      ItalicFont=NewCM08-BookItalic.otf,%
      BoldFont=NewCM10-Bold.otf,%
      BoldItalicFont=NewCM10-BoldItalic.otf,%
      SlantedFont=NewCM08-Book.otf,%
      BoldSlantedFont=NewCM10-Bold.otf,%
      SmallCapsFeatures={Numbers=OldStyle}},
{Size= 9-, Font = NewCM10-Book.otf,
      ItalicFont=NewCM10-BookItalic.otf,%
      BoldFont=NewCM10-Bold.otf,%
      BoldItalicFont=NewCM10-BoldItalic.otf,%
      SlantedFont=NewCM10-Book.otf,%
      BoldSlantedFont=NewCM10-Bold.otf,%
      SmallCapsFeatures={Numbers=OldStyle}}%
  },%
  SmallCapsFeatures={Numbers=OldStyle},%
  BoldSlantedFont=NewCM10-Bold.otf,%
  SlantedFont=NewCM10-Book.otf,%
  BoldItalicFont=NewCM10-BoldItalic.otf,%
  BoldFont=NewCM10-Bold.otf,%
  ItalicFont=NewCM10-BookItalic.otf,%
  SlantedFeatures={FakeSlant=0.25},%
  BoldSlantedFeatures={FakeSlant=0.25},%
]{NewCM10-Book.otf}
\setsansfont[%
    SizeFeatures={%
{Size= -8, Font=NewCMSans08-Book.otf,%
           ItalicFont=NewCMSans08-BookOblique.otf,%
           BoldFont=NewCMSans10-Bold.otf,%
           BoldItalicFont=NewCMSans10-BoldOblique.otf,%
           SmallCapsFeatures={Numbers=OldStyle},%
},
{Size= 8, Font=NewCMSans08-Book.otf,%
          ItalicFont=NewCMSans08-BookOblique.otf,%
          BoldFont=NewCMSans10-Bold.otf,%
          BoldItalicFont=NewCMSans10-BoldOblique.otf,%
          SmallCapsFeatures={Numbers=OldStyle},%
},
{Size= 9-, Font=NewCMSans10-Book.otf,%
           ItalicFont=NewCMSans10-BookOblique.otf,%
           BoldFont=NewCMSans10-Bold.otf,%
           BoldItalicFont=NewCMSans10-BoldOblique.otf,%
           SmallCapsFeatures={Numbers=OldStyle},%
}},
           ItalicFont=NewCMSans10-BookOblique.otf,%
           BoldFont=NewCMSans10-Bold.otf,%
           BoldItalicFont=NewCMSans10-BoldOblique.otf,%
           SmallCapsFeatures={Numbers=OldStyle},%
           SlantedFont=NewCMSans10-BookOblique.otf,%
           BoldSlantedFont=NewCMSans10-BoldOblique.otf,%
]{NewCMSans10-Book.otf}
\setmonofont[%
ItalicFont=NewCMMono10-BookItalic.otf,%
BoldFont=NewCMMono10-Bold.otf,%
BoldItalicFont=NewCMMono10-BoldOblique.otf,%
SlantedFont=NewCMMono10-Book.otf,%
SlantedFeatures={FakeSlant=0.25},
BoldSlantedFont=NewCMMono10-Bold.otf,%
BoldSlantedFeatures={FakeSlant=0.25},
SmallCapsFeatures={Numbers=OldStyle}]{NewCMMono10-Book.otf}
\newfontfamily\uncial[%
  SizeFeatures={%
{Size=-8, Font=NewCMUncial08-Book.otf,
      BoldFont=NewCMUncial10-Bold.otf,%
      SlantedFont=NewCMUncial08-Book.otf,%
      BoldSlantedFont=NewCMUncial10-Bold.otf,%
      },
{Size=8, Font=NewCMUncial08-Book.otf,
      BoldFont=NewCMUncial08-Bold.otf,%
      SlantedFont=NewCMUncial08-Book.otf,%
      BoldSlantedFont=NewCMUncial10-Bold.otf,%
      },
{Size= 9-, Font = NewCMUncial10-Book.otf,
      BoldFont=NewCMUncial10-Bold.otf,%
      SlantedFont=NewCMUncial10-Book.otf,%
      BoldSlantedFont=NewCMUncial10-Bold.otf,%
      }%
  },%
  BoldSlantedFont=NewCMUncial10-Bold.otf,%
  SlantedFont=NewCMUncial10-Book.otf,%
  BoldFont=NewCMUncial10-Bold.otf,%
  SlantedFeatures={FakeSlant=0.25},%
  BoldSlantedFeatures={FakeSlant=0.25},%
  ]{NewCMUncial10-Book.otf}
\newcommand{\textuncial}[1]{{\uncial #1}}
\setmathfont{NewCMMath-Book.otf}
\setmathfont{NewCMMath-Bold.otf}[version=bold]
\setmathfont[range={\mathscr,\mathbfscr},StylisticSet=1]{NewCMMath-Book.otf}
\newcommand{\tttextsc}[1]{{\ttscshape#1}}
%
\let\prosgegrammeni=\undefined
\newcommand{\prosgegrammeni}{\addfontfeature{StylisticSet=1}}
\newcommand{\textprosgegrammeni}[1]{{\prosgegrammeni#1}}
%
%\newfontfamily{\ivbce}[StylisticSet=2]{NewCMSans10-Book.otf}
\newcommand{\ivbce}{\sffamily\addfontfeature{StylisticSet=2}}
\newcommand{\textivbce}[1]{{\ivbce#1}}
%
%\newfontfamily{\ivbcealt}[StylisticSet=3]{NewCMSans10-Book.otf}
\newcommand{\ivbcealt}{\sffamily\addfontfeature{StylisticSet=3}}
\newcommand{\textivbcealt}[1]{{\ivbcealt#1}}
%
%\newfontfamily{\vibce}[StylisticSet=4]{NewCMSans10-Book.otf}
\newcommand{\vibce}{\sffamily\addfontfeature{StylisticSet=4}}
\newcommand{\textvibce}[1]{{\vibce#1}}
%
%% math (upright) sans Greek
\newcommand*{\msansAlpha}{\char"E000}
\newcommand*{\msansBeta}{\char"E001}
\newcommand*{\msansGamma}{\char"E002}
\newcommand*{\msansDelta}{\char"E003}
\newcommand*{\msansEpsilon}{\char"E004}
\newcommand*{\msansZeta}{\char"E005}
\newcommand*{\msansEta}{\char"E006}
\newcommand*{\msansTheta}{\char"E007}
\newcommand*{\msansIota}{\char"E008}
\newcommand*{\msansKappa}{\char"E009}
\newcommand*{\msansLambda}{\char"E00A}
\newcommand*{\msansMu}{\char"E00B}
\newcommand*{\msansNu}{\char"E00C}
\newcommand*{\msansXi}{\char"E00D}
\newcommand*{\msansOmicron}{\char"E00E}
\newcommand*{\msansPi}{\char"E00F}
\newcommand*{\msansRho}{\char"E010}
\newcommand*{\msansSigma}{\char"E011}
\newcommand*{\msansTau}{\char"E012}
\newcommand*{\msansUpsilon}{\char"E013}
\newcommand*{\msansPhi}{\char"E014}
\newcommand*{\msansChi}{\char"E015}
\newcommand*{\msansPsi}{\char"E016}
\newcommand*{\msansOmega}{\char"E017}
\newcommand*{\msansalpha}{\char"E018}
\newcommand*{\msansbeta}{\char"E019}
\newcommand*{\msansgamma}{\char"E01A}
\newcommand*{\msansdelta}{\char"E01B}
\newcommand*{\msansepsilon}{\char"E01C}
\newcommand*{\msanszeta}{\char"E01D}
\newcommand*{\msanseta}{\char"E01E}
\newcommand*{\msanstheta}{\char"E01F}
\newcommand*{\msansiota}{\char"E020}
\newcommand*{\msanskappa}{\char"E021}
\newcommand*{\msanslambda}{\char"E022}
\newcommand*{\msansmu}{\char"E023}
\newcommand*{\msansnu}{\char"E024}
\newcommand*{\msansxi}{\char"E025}
\newcommand*{\msansomicron}{\char"E026}
\newcommand*{\msanspi}{\char"E027}
\newcommand*{\msansrho}{\char"E028}
\newcommand*{\msansvarsigma}{\char"E029}
\newcommand*{\msanssigma}{\char"E02A}
\newcommand*{\msanstau}{\char"E02B}
\newcommand*{\msansupsilon}{\char"E02C}
\newcommand*{\msansphi}{\char"E02D}
\newcommand*{\msanschi}{\char"E02E}
\newcommand*{\msanspsi}{\char"E02F}
\newcommand*{\msansomega}{\char"E030}
\newcommand*{\msansvarepsilon}{\char"E031}
% math italic sans Greek
\newcommand*{\mitsansAlpha}{\char"E041}
\newcommand*{\mitsansBeta}{\char"E042}
\newcommand*{\mitsansGamma}{\char"E043}
\newcommand*{\mitsansDelta}{\char"E044}
\newcommand*{\mitsansEpsilon}{\char"E045}
\newcommand*{\mitsansZeta}{\char"E046}
\newcommand*{\mitsansEta}{\char"E047}
\newcommand*{\mitsansTheta}{\char"E048}
\newcommand*{\mitsansIota}{\char"E049}
\newcommand*{\mitsansKappa}{\char"E04A}
\newcommand*{\mitsansLambda}{\char"E04B}
\newcommand*{\mitsansMu}{\char"E04C}
\newcommand*{\mitsansNu}{\char"E04D}
\newcommand*{\mitsansXi}{\char"E04E}
\newcommand*{\mitsansOmicron}{\char"E04F}
\newcommand*{\mitsansPi}{\char"E050}
\newcommand*{\mitsansRho}{\char"E051}
\newcommand*{\mitsansSigma}{\char"E052}
\newcommand*{\mitsansTau}{\char"E053}
\newcommand*{\mitsansUpsilon}{\char"E054}
\newcommand*{\mitsansPhi}{\char"E055}
\newcommand*{\mitsansChi}{\char"E056}
\newcommand*{\mitsansPsi}{\char"E057}
\newcommand*{\mitsansOmega}{\char"E058}
\newcommand*{\mitsansalpha}{\char"E059}
\newcommand*{\mitsansbeta}{\char"E05A}
\newcommand*{\mitsansgamma}{\char"E05B}
\newcommand*{\mitsansdelta}{\char"E05C}
\newcommand*{\mitsansepsilon}{\char"E05D}
\newcommand*{\mitsanszeta}{\char"E05E}
\newcommand*{\mitsanseta}{\char"E05F}
\newcommand*{\mitsanstheta}{\char"E060}
\newcommand*{\mitsansiota}{\char"E061}
\newcommand*{\mitsanskappa}{\char"E062}
\newcommand*{\mitsanslambda}{\char"E063}
\newcommand*{\mitsansmu}{\char"E064}
\newcommand*{\mitsansnu}{\char"E065}
\newcommand*{\mitsansxi}{\char"E066}
\newcommand*{\mitsansomicron}{\char"E067}
\newcommand*{\mitsanspi}{\char"E068}
\newcommand*{\mitsansrho}{\char"E069}
\newcommand*{\mitsansvarsigma}{\char"E06A}
\newcommand*{\mitsanssigma}{\char"E06B}
\newcommand*{\mitsanstau}{\char"E06C}
\newcommand*{\mitsansupsilon}{\char"E06D}
\newcommand*{\mitsansphi}{\char"E06E}
\newcommand*{\mitsanschi}{\char"E06F}
\newcommand*{\mitsanspsi}{\char"E070}
\newcommand*{\mitsansomega}{\char"E071}
\newcommand*{\mitsansvarepsilon}{\char"E072}
% Ancient Greek Numerals u10140-u1018E
\newcommand*{\atticonequarter}{\char"10140}
\newcommand*{\atticonehalf}{\char"10141}
\newcommand*{\atticonedrachma}{\char"10142}
\newcommand*{\atticfive}{\char"10143}
\newcommand*{\atticfifty}{\char"10144}
\newcommand*{\atticfivehundred}{\char"10145}
\newcommand*{\atticfivethousand}{\char"10146}
\newcommand*{\atticfiftythousand}{\char"10147}
\newcommand*{\atticfivetalents}{\char"10148}
\newcommand*{\attictentalents}{\char"10149}
\newcommand*{\atticfiftytalents}{\char"1014A}
\newcommand*{\atticonehundredtalents}{\char"1014B}
\newcommand*{\atticfivehundredtalents}{\char"1014C}
\newcommand*{\atticonethousandtalents}{\char"1014D}
\newcommand*{\atticfivethousandtalents}{\char"1014E}
\newcommand*{\atticfivestaters}{\char"1014F}
\newcommand*{\attictenstaters}{\char"10150}
\newcommand*{\atticfiftystaters}{\char"10151}
\newcommand*{\atticonehundredstaters}{\char"10152}
\newcommand*{\atticfivehundredstaters}{\char"10153}
\newcommand*{\atticonethousandstaters}{\char"10154}
\newcommand*{\attictenthousandstaters}{\char"10155}
\newcommand*{\atticfiftythousandstaters}{\char"10156}
\newcommand*{\attictenmnas}{\char"10157}
\newcommand*{\heraleumoneplethron}{\char"10158}
\newcommand*{\thespianone}{\char"10159}
\newcommand*{\ermionianone}{\char"1015A}
\newcommand*{\epidauriantwo}{\char"1015B}
\newcommand*{\thespiantwo}{\char"1015C}
\newcommand*{\cyrenaictwodrachmas}{\char"1015D}
\newcommand*{\epidauriantwodrachmas}{\char"1015E}
\newcommand*{\troezenianfive}{\char"1015F}
\newcommand*{\troezenianten}{\char"10160}
\newcommand*{\troezeniantenalt}{\char"10161}
\newcommand*{\hermionianten}{\char"10162}
\newcommand*{\messenianten}{\char"10163}
\newcommand*{\thespianten}{\char"10164}
\newcommand*{\thespianthirty}{\char"10165}
\newcommand*{\troezenianfifty}{\char"10166}
\newcommand*{\troezenianfiftyalt}{\char"10167}
\newcommand*{\hermionianfifty}{\char"10168}
\newcommand*{\thespianfifty}{\char"10169}
\newcommand*{\thespianonehundred}{\char"1016A}
\newcommand*{\thespianthreehundred}{\char"1016B}
\newcommand*{\epidaurianfivehundred}{\char"1016C}
\newcommand*{\troezenianfivehundred}{\char"1016D}
\newcommand*{\thespianfivehundred}{\char"1016E}
\newcommand*{\carystianfivehundred}{\char"1016F}
\newcommand*{\naxianfivehundred}{\char"10170}
\newcommand*{\thespianonethousand}{\char"10171}
\newcommand*{\thespianfivethousand}{\char"10172}
\newcommand*{\delphicfivemnas}{\char"10173}
\newcommand*{\stratianfiftymnas}{\char"10174}
\newcommand*{\greekonehalfsign}{\char"10175}
\newcommand*{\greekonehalfsignalt}{\char"10176}
\newcommand*{\greektwothirdssign}{\char"10177}
\newcommand*{\greekthreequarterssign}{\char"10178}
\newcommand*{\greekyearsign}{\char"10179}
\newcommand*{\greektalentsign}{\char"1017A}
\newcommand*{\greekdrachmasign}{\char"1017B}
\newcommand*{\greekobolsign}{\char"1017C}
\newcommand*{\greektwoobolssign}{\char"1017D}
\newcommand*{\greekthreeobolssign}{\char"1017E}
\newcommand*{\greekfourobolssign}{\char"1017F}
\newcommand*{\greekfiveobolssign}{\char"10180}
\newcommand*{\greekmetretessign}{\char"10181}
\newcommand*{\greekkyathosbasesign}{\char"10182}
\newcommand*{\greeklytrasign}{\char"10183}
\newcommand*{\greekounkiasign}{\char"10184}
\newcommand*{\greekxestessign}{\char"10185}
\newcommand*{\greekartabesign}{\char"10186}
\newcommand*{\greekarourasign}{\char"10187}
\newcommand*{\greekgrammasign}{\char"10188}
\newcommand*{\greektryblionbasesign}{\char"10189}
\newcommand*{\greekzerosign}{\char"1018A}
\newcommand*{\greekonequartersign}{\char"1018B}
\newcommand*{\greeksinusoidsign}{\char"1018C}
\newcommand*{\greekindictionsign}{\char"1018D}
\newcommand*{\nomismasign}{\char"1018E}
%
% some math symbols
\DeclareRobustCommand*\nrightrightarrows{\mathrel{\char"E033}}
\DeclareRobustCommand*\nleftleftarrows{\mathrel{\char"E032}}
\DeclareRobustCommand*\twoheadhookrightarrow{\mathrel{\char"E034}}
\DeclareRobustCommand*\twoheadhookleftarrow{\mathrel{\char"E035}}
%
%%% declare the convolution operator %%%%%%%%%%%%%%%
\DeclareMathOperator*{\convolution}{\mathchoice{\char"E037}{\char"E036}{\char"E038}{\char"E039}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% select ss02 lookup table for IPA symbols
%\newfontfamily{\ipatext}[StylisticSet=5,%
%BoldFont=NewCM10-Bold.otf,%
%SlantedFont=NewCM10-Regular.otf,%
%SlantedFeatures={FakeSlant=0.25},
%BoldSlantedFont=NewCM10-Bold.otf,%
%BoldSlantedFeatures={FakeSlant=0.25},
%SmallCapsFeatures={Numbers=OldStyle}]{NewCM10-Book.otf}
\newcommand{\ipatext}{\addfontfeature{StylisticSet=5}}
\newcommand{\textipa}[1]{{\ipatext#1}}
\newcommand{\oldipatext}{\addfontfeature{StylisticSet=5,RawFeature=+lipa}}
\newcommand{\textoldipa}[1]{{\oldipatext#1}}
%\newfontfamily{\ipatextsans}[StylisticSet=5,%
%ItalicFont=NewCMSans10-BookOblique.otf,%
%BoldFont=NewCMSans10-Bold.otf,%
%BoldItalicFont=NewCMSans10-BoldOblique.otf,%
%SlantedFont=NewCMSans10-Oblique.otf,%
%BoldSlantedFont=NewCMSans10-BoldOblique.otf,%
%SmallCapsFeatures={Numbers=OldStyle}]{NewCMSans10-Book.otf}
%\newcommand{\ipatextsans}{\sffamily\addfontfeature{StylisticSet=5}}
%\newcommand{\textsansipa}[1]{{\ipatextsans#1}}
%
% Up versions for chemistry
\newcommand*{\chemalpha}{\textrm{α}}
\newcommand*{\chembeta}{\textrm{β}}
\newcommand*{\chemgamma}{\textrm{γ}}
\newcommand*{\chemdelta}{\textrm{δ}}
\newcommand*{\chemepsilon}{\textrm{ε}}
\newcommand*{\chemzeta}{\textrm{ζ}}
\newcommand*{\chemeta}{\textrm{η}}
\newcommand*{\chemtheta}{\textrm{θ}}
\newcommand*{\chemiota}{\textrm{ι}}
\newcommand*{\chemkappa}{\textrm{\char"03F0}}
\newcommand*{\chemlambda}{\textrm{λ}}
\newcommand*{\chemmu}{\textrm{μ}}
\newcommand*{\chemnu}{\textrm{ν}}
\newcommand*{\chemxi}{\textrm{ξ}}
\newcommand*{\chemomicron}{\textrm{ο}}
\newcommand*{\chempi}{\textrm{π}}
\newcommand*{\chemrho}{\textrm{ρ}}
\newcommand*{\chemrhoalt}{\textrm{\char"03F1}}
\newcommand*{\chemsigma}{\textrm{σ}}
\newcommand*{\chemsigmaalt}{\textrm{ς}}
\newcommand*{\chemtau}{\textrm{τ}}
\newcommand*{\chemupsilon}{\textrm{υ}}
\newcommand*{\chemphi}{\textrm{φ}}
\newcommand*{\chemchi}{\textrm{χ}}
\newcommand*{\chempsi}{\textrm{ψ}}
\newcommand*{\chemomega}{\textrm{ω}}
%
\newcommand*{\chemAlpha}{\textrm{Α}}
\newcommand*{\chemBeta}{\textrm{Β}}
\newcommand*{\chemGamma}{\textrm{Γ}}
\newcommand*{\chemDelta}{\textrm{Δ}}
\newcommand*{\chemEpsilon}{\textrm{Ε}}
\newcommand*{\chemZeta}{\textrm{Ζ}}
\newcommand*{\chemEta}{\textrm{Η}}
\newcommand*{\chemTheta}{\textrm{Θ}}
\newcommand*{\chemIota}{\textrm{Ι}}
\newcommand*{\chemKappa}{\textrm{Κ}}
\newcommand*{\chemLambda}{\textrm{Λ}}
\newcommand*{\chemMu}{\textrm{Μ}}
\newcommand*{\chemNu}{\textrm{Ν}}
\newcommand*{\chemXi}{\textrm{Ξ}}
\newcommand*{\chemOmicron}{\textrm{Ο}}
\newcommand*{\chemPi}{\textrm{Π}}
\newcommand*{\chemRho}{\textrm{Ρ}}
\newcommand*{\chemSigma}{\textrm{Σ}}
\newcommand*{\chemTau}{\textrm{Τ}}
\newcommand*{\chemUpsilon}{\textrm{Υ}}
\newcommand*{\chemPhi}{\textrm{Φ}}
\newcommand*{\chemChi}{\textrm{Χ}}
\newcommand*{\chemPsi}{\textrm{Ψ}}
\newcommand*{\chemOmega}{\textrm{Ω}}
%
%% Next block enables Devanagari letters as variables in Math font
\Umathcode "0900 7 \symoperators "0900%
\Umathcode "0901 7 \symoperators "0901%
\Umathcode "0902 7 \symoperators "0902%
\Umathcode "0903 7 \symoperators "0903%
\Umathcode "0904 7 \symoperators "0904%
\Umathcode "0905 7 \symoperators "0905%
\Umathcode "0906 7 \symoperators "0906%
\Umathcode "0907 7 \symoperators "0907%
\Umathcode "0908 7 \symoperators "0908%
\Umathcode "0909 7 \symoperators "0909%
\Umathcode "090A 7 \symoperators "090A%
\Umathcode "090B 7 \symoperators "090B%
\Umathcode "090C 7 \symoperators "090C%
\Umathcode "090D 7 \symoperators "090D%
\Umathcode "090E 7 \symoperators "090E%
\Umathcode "090F 7 \symoperators "090F%
%
\Umathcode "0910 7 \symoperators "0910%
\Umathcode "0911 7 \symoperators "0911%
\Umathcode "0912 7 \symoperators "0912%
\Umathcode "0913 7 \symoperators "0913%
\Umathcode "0914 7 \symoperators "0914%
\Umathcode "0915 7 \symoperators "0915%
\Umathcode "0916 7 \symoperators "0916%
\Umathcode "0917 7 \symoperators "0917%
\Umathcode "0918 7 \symoperators "0918%
\Umathcode "0919 7 \symoperators "0919%
\Umathcode "091A 7 \symoperators "091A%
\Umathcode "091B 7 \symoperators "091B%
\Umathcode "091C 7 \symoperators "091C%
\Umathcode "091D 7 \symoperators "091D%
\Umathcode "091E 7 \symoperators "091E%
\Umathcode "091F 7 \symoperators "091F%
%
\Umathcode "0920 7 \symoperators "0920%
\Umathcode "0921 7 \symoperators "0921%
\Umathcode "0922 7 \symoperators "0922%
\Umathcode "0923 7 \symoperators "0923%
\Umathcode "0924 7 \symoperators "0924%
\Umathcode "0925 7 \symoperators "0925%
\Umathcode "0926 7 \symoperators "0926%
\Umathcode "0927 7 \symoperators "0927%
\Umathcode "0928 7 \symoperators "0928%
\Umathcode "0929 7 \symoperators "0929%
\Umathcode "092A 7 \symoperators "092A%
\Umathcode "092B 7 \symoperators "092B%
\Umathcode "092C 7 \symoperators "092C%
\Umathcode "092D 7 \symoperators "092D%
\Umathcode "092E 7 \symoperators "092E%
\Umathcode "092F 7 \symoperators "092F%
%
\Umathcode "0930 7 \symoperators "0930%
\Umathcode "0931 7 \symoperators "0931%
\Umathcode "0932 7 \symoperators "0932%
\Umathcode "0933 7 \symoperators "0933%
\Umathcode "0934 7 \symoperators "0934%
\Umathcode "0935 7 \symoperators "0935%
\Umathcode "0936 7 \symoperators "0936%
\Umathcode "0937 7 \symoperators "0937%
\Umathcode "0938 7 \symoperators "0938%
\Umathcode "0939 7 \symoperators "0939%
\Umathcode "093A 7 \symoperators "093A%
\Umathcode "093B 7 \symoperators "093B%
\Umathcode "093C 7 \symoperators "093C%
\Umathcode "093D 7 \symoperators "093D%
\Umathcode "093E 7 \symoperators "093E%
\Umathcode "093F 7 \symoperators "093F%
%
\Umathcode "0940 7 \symoperators "0940%
\Umathcode "0941 7 \symoperators "0941%
\Umathcode "0942 7 \symoperators "0942%
\Umathcode "0943 7 \symoperators "0943%
\Umathcode "0944 7 \symoperators "0944%
\Umathcode "0945 7 \symoperators "0945%
\Umathcode "0946 7 \symoperators "0946%
\Umathcode "0947 7 \symoperators "0947%
\Umathcode "0948 7 \symoperators "0948%
\Umathcode "0949 7 \symoperators "0949%
\Umathcode "094A 7 \symoperators "094A%
\Umathcode "094B 7 \symoperators "094B%
\Umathcode "094C 7 \symoperators "094C%
\Umathcode "094D 7 \symoperators "094D%
\Umathcode "094E 7 \symoperators "094E%
\Umathcode "094F 7 \symoperators "094F%
%
\Umathcode "0950 7 \symoperators "0950%
\Umathcode "0951 7 \symoperators "0951%
\Umathcode "0952 7 \symoperators "0952%
\Umathcode "0953 7 \symoperators "0953%
\Umathcode "0954 7 \symoperators "0954%
\Umathcode "0955 7 \symoperators "0955%
\Umathcode "0956 7 \symoperators "0956%
\Umathcode "0957 7 \symoperators "0957%
\Umathcode "0958 7 \symoperators "0958%
\Umathcode "0959 7 \symoperators "0959%
\Umathcode "095A 7 \symoperators "095A%
\Umathcode "095B 7 \symoperators "095B%
\Umathcode "095C 7 \symoperators "095C%
\Umathcode "095D 7 \symoperators "095D%
\Umathcode "095E 7 \symoperators "095E%
\Umathcode "095F 7 \symoperators "095F%
%
\Umathcode "0960 7 \symoperators "0960%
\Umathcode "0961 7 \symoperators "0961%
\Umathcode "0962 7 \symoperators "0962%
\Umathcode "0963 7 \symoperators "0963%
\Umathcode "0964 7 \symoperators "0964%
\Umathcode "0965 7 \symoperators "0965%
\Umathcode "0966 7 \symoperators "0966%
\Umathcode "0967 7 \symoperators "0967%
\Umathcode "0968 7 \symoperators "0968%
\Umathcode "0969 7 \symoperators "0969%
\Umathcode "096A 7 \symoperators "096A%
\Umathcode "096B 7 \symoperators "096B%
\Umathcode "096C 7 \symoperators "096C%
\Umathcode "096D 7 \symoperators "096D%
\Umathcode "096E 7 \symoperators "096E%
\Umathcode "096F 7 \symoperators "096F%
%
\Umathcode "0970 7 \symoperators "0970%
\Umathcode "0971 7 \symoperators "0971%
\Umathcode "0972 7 \symoperators "0972%
\Umathcode "0973 7 \symoperators "0973%
\Umathcode "0974 7 \symoperators "0974%
\Umathcode "0975 7 \symoperators "0975%
\Umathcode "0976 7 \symoperators "0976%
\Umathcode "0977 7 \symoperators "0977%
\Umathcode "0978 7 \symoperators "0978%
\Umathcode "0979 7 \symoperators "0979%
\Umathcode "097A 7 \symoperators "097A%
\Umathcode "097B 7 \symoperators "097B%
\Umathcode "097C 7 \symoperators "097C%
\Umathcode "097D 7 \symoperators "097D%
\Umathcode "097E 7 \symoperators "097E%
\Umathcode "097F 7 \symoperators "097F%
%\Umathcode `ज 7 \symoperators "091C%
%\Umathcode `अ 7 \symoperators "0905%
%\Umathcode "0905 7 \symoperators "0905%
%\Umathcode `क 7 \symoperators "0915%
%\Umathcode `ख 7 \symoperators "0916%
%\Umathcode `२ 7 \symoperators "0968%
%\count255="0900
% \loop\ifnum\count255<"097F
%   \advance\count255 by 1
%   \Umathcode \count255 7 \symoperators \count255\fi
% \repeat
%%%%%%%%%%%%%%% End Devanagari Variables block %%%%%%%%


%%%%%%%%%% Begin Aegean Numbers #######################
\newcommand*{\aegeanseparator}{\textsf{\char"10100}}
\newcommand*{\aegeanseparatordot}{\textsf{\char"10101}}
\newcommand*{\aegeancheckmark}{\textsf{\char"10102}}
\newcommand*{\aegeanone}{\textsf{\char"10107}}
\newcommand*{\aegeantwo}{\textsf{\char"10108}}
\newcommand*{\aegeanthree}{\textsf{\char"10109}}
\newcommand*{\aegeanfour}{\textsf{\char"1010A}}
\newcommand*{\aegeanfive}{\textsf{\char"1010B}}
\newcommand*{\aegeansix}{\textsf{\char"1010C}}
\newcommand*{\aegeanseven}{\textsf{\char"1010D}}
\newcommand*{\aegeaneight}{\textsf{\char"1010E}}
\newcommand*{\aegeanine}{\textsf{\char"1010F}}
\newcommand*{\aegeanten}{\textsf{\char"10110}}
\newcommand*{\aegeantwenty}{\textsf{\char"10111}}
\newcommand*{\aegeanthirty}{\textsf{\char"10112}}
\newcommand*{\aegeanfourty}{\textsf{\char"10113}}
\newcommand*{\aegeanfifty}{\textsf{\char"10114}}
\newcommand*{\aegeansixty}{\textsf{\char"10115}}
\newcommand*{\aegeanseventy}{\textsf{\char"10116}}
\newcommand*{\aegeaneighty}{\textsf{\char"10117}}
\newcommand*{\aegeanninety}{\textsf{\char"10118}}
\newcommand*{\aegeanonehundred}{\textsf{\char"10119}}
\newcommand*{\aegeantwohundred}{\textsf{\char"1011A}}
\newcommand*{\aegeanthreehundred}{\textsf{\char"1011B}}
\newcommand*{\aegeanfourhundred}{\textsf{\char"1011C}}
\newcommand*{\aegeanfivehundred}{\textsf{\char"1011D}}
\newcommand*{\aegeansixhundred}{\textsf{\char"1011E}}
\newcommand*{\aegeansevenhundred}{\textsf{\char"1011F}}
\newcommand*{\aegeaneighthundred}{\textsf{\char"10120}}
\newcommand*{\aegeanninehundred}{\textsf{\char"10121}}
\newcommand*{\aegeanonethousand}{\textsf{\char"10122}}
\newcommand*{\aegeantwothousand}{\textsf{\char"10123}}
\newcommand*{\aegeanthreethousand}{\textsf{\char"10124}}
\newcommand*{\aegeanfourthousand}{\textsf{\char"10125}}
\newcommand*{\aegeanfivethousand}{\textsf{\char"10126}}
\newcommand*{\aegeansixthousand}{\textsf{\char"10127}}
\newcommand*{\aegeanseventhousand}{\textsf{\char"10128}}
\newcommand*{\aegeaneightthousand}{\textsf{\char"10129}}
\newcommand*{\aegeanninethousand}{\textsf{\char"1012A}}
\newcommand*{\aegeantenthousand}{\textsf{\char"1012B}}
\newcommand*{\aegeantwentythousand}{\textsf{\char"1012C}}
\newcommand*{\aegeanthirtythousand}{\textsf{\char"1012D}}
\newcommand*{\aegeanfourtythousand}{\textsf{\char"1012E}}
\newcommand*{\aegeanfiftythousand}{\textsf{\char"1012F}}
\newcommand*{\aegeansixtythousand}{\textsf{\char"10130}}
\newcommand*{\aegeanseventythousand}{\textsf{\char"10131}}
\newcommand*{\aegeaneightythousand}{\textsf{\char"10132}}
\newcommand*{\aegeanninetythousand}{\textsf{\char"10133}}
\newcommand*{\aegeanweightbaseunit}{\textsf{\char"10137}}
\newcommand*{\aegeanweightfirstsubunit}{\textsf{\char"10138}}
\newcommand*{\aegeanweightsecondsubunit}{\textsf{\char"10139}}
\newcommand*{\aegeanweightthirdsubunit}{\textsf{\char"1013A}}
\newcommand*{\aegeanweightfourthsubunit}{\textsf{\char"1013B}}
\newcommand*{\aegeandrymeasurefirstsubunit}{\textsf{\char"1013C}}
\newcommand*{\aegeanliquidmeasurefirstsubunit}{\textsf{\char"1013D}}
\newcommand*{\aegeansecondsubunit}{\textsf{\char"1013E}}
\newcommand*{\aegeanthirdsubunit}{\textsf{\char"1013F}}
%%%%%%%%%%%%%%%% End Aegean Numbers %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\endinput

